Gender Differences in Participation and Reward on Stack Overflow

Programming is a valuable skill in the labor market, making the underrepresentation of women in computing an increasingly important issue. Online question and answer platforms serve a dual purpose in this field: they form a body of knowledge useful as a reference and learning tool, and they provide opportunities for individuals to demonstrate credible, verifiable expertise. Issues, such as male-oriented site design or overrepresentation of men among the site's elite may therefore compound the issue of women's underrepresentation in IT. In this paper we audit the differences in behavior and outcomes between men and women on Stack Overflow, the most popular of these Q&A sites. We observe significant differences in how men and women participate in the platform and how successful they are. For example, the average woman has roughly half of the reputation points, the primary measure of success on the site, of the average man. Using an Oaxaca-Blinder decomposition, an econometric technique commonly applied to analyze differences in wages between groups, we find that most of the gap in success between men and women can be explained by differences in their activity on the site and differences in how these activities are rewarded. Specifically, 1) men give more answers than women and 2) are rewarded more for their answers on average, even when controlling for possible confounders such as tenure or buy-in to the site. Women ask more questions and gain more reward per question. We conclude with a hypothetical redesign of the site's scoring system based on these behavioral differences, cutting the reputation gap in half.

==> app.tex <==
\section{Appendix}

\begin{figure}[b]
  \includegraphics[width=0.75\columnwidth]{figures/interaction_neutral.png}
  \caption{User reputation regressed on activity on the platform, controlling for self-promotion indicators and community-level features. The distinct colors and fitted curves denote regressions ran for women, men and unidentified users separately. The difference in slopes between women and men indicates that men get more reputation points for additional answers. The slope of the unidentified users' curve is in between men's and women's showing that the characteristics of these users fall between those of the identified men's and women's.}
  \label{selfpromotion}
\end{figure}

\begin{table*}
\centering 
\begin{tabular}{lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable: $\ln(\mathrm{Reputation})$}} \\ 
\\[-1.8ex] & Male users & Female users & Uncategorized users\\ 
\hline \\[-1.8ex] 
 Answers Posted & 0.58$^{***}$ (0.01) & 0.45$^{***}$ (0.01) & 0.52$^{***}$ (0.01) \\ 
 Questions Posted & 0.07$^{***}$ (0.005) & 0.10$^{***}$ (0.01) & 0.09$^{***}$ (0.005) \\ 
 Votes Casted & 0.09$^{***}$ (0.004) & 0.07$^{***}$ (0.01) & 0.10$^{***}$ (0.004) \\
 Account Age & 0.53$^{***}$ (0.01) & 0.46$^{***}$ (0.01) & 0.54$^{***}$ (0.01) \\ 
 Self-promotion Controls & YES & YES & YES \\ 
 Community Controls & YES & YES & YES \\ 
 Constant & 0.78$^{**}$ (0.38) & 1.73$^{***}$ (0.50) & 1.35$^{***}$ (0.39) \\
\hline \\[-1.8ex] 
Observations & 19,728 & 10,571 & 19,248 \\ 
R$^{2}$ & 0.67 & 0.56 & 0.63 \\ 
Residual Std. Error & 0.74 & 0.72 & 0.73 \\ 
F Statistic & 2,150.20$^{***}$ & 694.85$^{***}$ & 1,712.00$^{***}$ \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\bigskip
 \caption{Regression 3 (see Table 4) repeated for the users with identified genders and unidentified ones separately. In each case, users' reputation is regressed on user-level activity measures, controlling for self-promotion indicators and community-level features. The coefficients from the model of the unidentified users fall between the coefficients of the men and women, which suggests that the unidentified observations are not different from the identified ones in terms of the relationship between their activity and success. \textit{Note:}  $^{*}p < 0.1$; $^{**}p < 0.05$; $^{***}p < 0.01$}
 \label{interactiontable_neutral} 
\end{table*}


==> reg_inter.tex <==

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: sze, okt 04, 2017 - 22:30:51
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{ln\_rep} \\ 
 & baseline & many class contr & many class contr + inter \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 male & 0.02$^{***}$ & 0.02$^{***}$ & $-$0.15$^{***}$ \\ 
  & (0.01) & (0.01) & (0.01) \\ 
  & & & \\ 
 ln\_nanswers & 0.52$^{***}$ & 0.53$^{***}$ & 0.49$^{***}$ \\ 
  & (0.003) & (0.003) & (0.004) \\ 
  & & & \\ 
 ln\_nquestions & 0.08$^{***}$ & 0.09$^{***}$ & 0.09$^{***}$ \\ 
  & (0.003) & (0.003) & (0.004) \\ 
  & & & \\ 
 ln\_votes\_cast & 0.09$^{***}$ & 0.09$^{***}$ & 0.09$^{***}$ \\ 
  & (0.003) & (0.003) & (0.003) \\ 
  & & & \\ 
 ln\_account\_age\_days & 0.51$^{***}$ & 0.52$^{***}$ & 0.52$^{***}$ \\ 
  & (0.01) & (0.01) & (0.01) \\ 
  & & & \\ 
 self\_promote &  & $-$0.003 & $-$0.01 \\ 
  &  & (0.01) & (0.01) \\ 
  & & & \\ 
 leader &  & 0.07$^{***}$ & 0.06$^{***}$ \\ 
  &  & (0.02) & (0.02) \\ 
  & & & \\ 
 male:ln\_nanswers &  &  & 0.09$^{***}$ \\ 
  &  &  & (0.005) \\ 
  & & & \\ 
 male:ln\_nquestions &  &  & $-$0.02$^{***}$ \\ 
  &  &  & (0.005) \\ 
  & & & \\ 
 Constant & 0.57$^{***}$ & 1.62$^{***}$ & 1.70$^{***}$ \\ 
  & (0.05) & (0.26) & (0.26) \\ 
  & & & \\ 
\hline \\[-1.8ex] 
Observations & 49,570 & 49,570 & 49,570 \\ 
R$^{2}$ & 0.63 & 0.64 & 0.64 \\ 
Adjusted R$^{2}$ & 0.63 & 0.64 & 0.64 \\ 
Residual Std. Error & 0.74 (df = 49564) & 0.74 (df = 49549) & 0.74 (df = 49547) \\ 
F Statistic & 16,938.67$^{***}$ (df = 5; 49564) & 4,339.10$^{***}$ (df = 20; 49549) & 3,986.34$^{***}$ (df = 22; 49547) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

